Proof Nets and the Linear Substitution Calculus

Since the very beginning of the theory of linear logic it is known how to represent the $\lambda$-calculus as linear logic proof nets. The two systems however have different granularities, in particular proof nets have an explicit notion of sharing---the exponentials---and a micro-step operational semantics, while the $\lambda$-calculus has no sharing and a small-step operational semantics. Here we show that the \emph{linear substitution calculus}, a simple refinement of the $\lambda$-calculus with sharing, is isomorphic to proof nets at the operational level. Nonetheless, two different terms with sharing can still have the same proof nets representation---a further result is the characterisation of the equality induced by proof nets over terms with sharing. Finally, such a detailed analysis of the relationship between terms and proof nets, suggests a new, abstract notion of proof net, based on rewriting considerations and not necessarily of a graphical nature.

==> macros/graphical-macros/boxes.tex <==
\newcommand{\stboxlw}{6pt}
\newcommand{\stboxh}{20pt}
\newcommand{\stboxrwaux}{35pt}
\newcommand{\stboxrw}{30pt}
\newcommand{\sepbox}{2pt}
\newcommand{\belowbox}{\stboxh+2*\sepbox+1pt}

\newcommand{\boxinit}{
\pgfdeclarelayer{background layer} 
\pgfdeclarelayer{foreground layer} 
\pgfsetlayers{background layer,main,foreground layer} 
}

\newcommand{\posboxlink}[3]{%parametri: #1=pos principal port, #2= link name, #3=actual pos link
\node at (#1.center) [above=\hstalt, fill=white, etic] (#2){#3};
\draw[posln] (#1) to (#2);
}

\newcommand{\posboxlinkm}[3]{%parametri: #1=pos principal port, #2= link name, #3=actual pos link
\node at (#1.center) [above=\hstaltm, fill=white, etic] (#2){\tiny #3};
\draw[posln] (#1) to (#2);
}

\newcommand{\posboxlinkmfake}[2]{%parametri: #1=pos principal port, #2= link name, 
\node at (#1.center) [above=\hstaltm-3pt, inner sep= 2pt] (#2){};
\draw[posln] (#1) to (#2);
}


\newcommand{\nopolboxlink}[3]{%parametri: #1=pos principal port, #2= link name, #3=actual pos link
\node at (#1.center) [above=\hstalt, fill=white, etic] (#2){#3};
\draw[nopolrev] (#1) to (#2);
}


\newcommand{\nopolboxlinkrev}[3]{%parametri: #1=pos principal port, #2= link name, #3=actual pos link
\node at (#1.center) [above=\hstalt, fill=white, etic] (#2){#3};
\draw[nopol] (#1) to (#2);
}

\newcommand{\boxline}[2]{%parametri: #1=box link, 2=line style
%\begin{pgfonlayer}{background layer} 
\draw[#2](#1.center) -- (#1se.center) -- (#1ne.center) -- (#1no.center) -- (#1so.center)--(#1.center); 
%\end{pgfonlayer}
}

\newcommand{\boxlineopenup}[2]{%parametri: #1=box link, 2=line style
\begin{pgfonlayer}{background layer} 
%\draw[#2](#1.center) -- (#1se.center) -- (#1ne.center) -- (#1no.center) -- (#1so.center)--(#1.center); 
\draw[#2](#1no.center) -- (#1so.center)--(#1se.center) -- (#1ne.center) ; 
\end{pgfonlayer}
}

\newcommand{\boxlinecorner}[2]{%parametri: #1=box link, 2=line style
\begin{pgfonlayer}{background layer} 
%\draw[#2](#1.center) -- (#1se.center) -- (#1ne.center) -- (#1no.center) -- (#1so.center)--(#1.center); 
\draw[#2] (#1so.center)--(#1se.center) -- (#1ne.center) ; 
\end{pgfonlayer}
}


\newcommand{\boxcornerright}[5]{%parameters: 1=link to box, 2=box kind, 3=box left width, 4=box right width, 5= box height, 
\boxnodes{#4}{#5}{#1}{#3}
\boxlinecorner{#1}{#2line}
}



\newcommand{\boxnodes}[4]{%parametri: #1=Larghezza box destra, %#2= altezza box, #3=link to box, 4=larghezza sinistra
\node at (#3.center)[left = #4,nospace](#3so){};
\node at (#3.center)[right = #1,nospace](#3se){};
\node at (#3se.center)[above=#2,nospace](#3ne){};
\node at (#3ne-|#3so)[nospace](#3no){};
}

\newcommand{\boxlabel}[2]{%parametri: #1=box link, 2=label
\node at ($(#1so)!.5!(#1ne)$) {#2};
}

\newcommand{\boxlabelnet}[2]{%parametri: #1=box link, 2=label
\node at ($(#1so)!.5!(#1ne)$) [smallnet] (#1lab){#2};
\draw[posnl, in =60, out=210](#1lab)to(#1);
}

\newcommand{\abox}[5]{%parameters: 1=link to box, 2=box kind, 3=box left width, 4=box right width, 5= box height, 
\boxnodes{#4}{#5}{#1}{#3}
\boxline{#1}{#2line}
}

\newcommand{\aboxopenup}[5]{%parameters: 1=link to box, 2=box kind, 3=box left width, 4=box right width, 5= box height, 
\boxnodes{#4}{#5}{#1}{#3}
\boxlineopenup{#1}{#2line}
}

\newcommand{\stbox}[2]{%parameters: 1=link to box, 2=box kind
\boxnodes{\stboxrw}{\stboxh}{#1}{\stboxlw}
\boxline{#1}{#2line}
}

\newcommand{\stboxaux}[2]{%parameters: 1=link to box, 2=box kind
\boxnodes{\stboxrwaux}{\stboxh}{#1}{\stboxlw}
\boxline{#1}{#2line}
}

\newcommand{\jaux}[2]{%parametri: 1=link to box, 2=box right width
\node at (#1se.center)[left = \stboxlw, negport](#1auxk){};
\node at (#1auxk.center)[left= ((#2)/2),negport](#1aux1){};
}

\newcommand{\jauxnoport}[2]{%parametri: 1=link to box, 2=box right width
\node at (#1se.center)[left = \stboxlw, nospace](#1auxnpk){};
\node at (#1auxnpk.center)[left= ((#2)/2),nospace](#1auxnp1){};
}
\newcommand{\jauxnoportshift}[3]{%parametri: 1=link to box, 2=box right width 3=shift
\node at (#1se.center)[left = \stboxlw+#3, nospace](#1auxnpk){};
\node at (#1auxnpk.center)[left= ((#2)/2),nospace](#1auxnp1){};
}


\newcommand{\jauxlab}[4]{%parametri: 1=link to box, 2=box right width, 3=left label, 4=right label
\node at (#1se.center)[left = \stboxlw, label=below:\tiny #4,negport](#1auxk){};
\node at (#1auxk.center)[left= ((#2)/2), label=below:\tiny #3,negport](#1aux1){};
\node at ($(#1aux1)!.5!(#1auxk)$)[below=2pt] {$\tiny\ldots$};
}

\newcommand{\iauxlab}[5]{%parametri: 1=link to box, 2=box right width, 3=left label, 4=right label, 5=height delta
\node at (#1se.center)[left = \stboxlw, negport](#1auxk){};
\node at (#1auxk.center)[left= ((#2)/2), negport](#1aux1){};
%\node at ($(#1aux1)!.5!(#1auxk)$)[below=2pt] {$\tiny\ldots$};
\node at (#1auxk.center)[below = #5, label= below:\tiny #4,negport](#1auxktarget){};
\node at (#1aux1.center)[below = #5, label= below:\tiny #3,negport](#1aux1target){};

\draw[negln] (#1auxk) to (#1auxktarget);
\draw[negln] (#1aux1) to (#1aux1target);
}

\newcommand{\iauxlabneutral}[5]{%parametri: 1=link to box, 2=box right width, 3=left label, 4=right label, 5=height delta
\node at (#1se.center)[left = \stboxlw, negport](#1auxk){};
\node at (#1auxk.center)[left= ((#2)/2), negport](#1aux1){};
%\node at ($(#1aux1)!.5!(#1auxk)$)[below=2pt] {$\tiny\ldots$};
\node at (#1auxk.center)[below = #5, label= below:\tiny #4,negport](#1auxktarget){};
\node at (#1aux1.center)[below = #5, label= below:\tiny #3,negport](#1aux1target){};

\draw[neutral] (#1auxk) to (#1auxktarget);
\draw[neutral] (#1aux1) to (#1aux1target);
}


\newcommand{\jauxlabh}[5]{%parametri: 1=link to box, 2=box right width, 3=left label, 4=right label, 5=height delta
\node at (#1se.center)[below left = #5 and \stboxlw, label=below:\tiny #4,negport](#1auxk){};
\node at (#1auxk.center)[left= ((#2)/2), label=below:\tiny #3,negport](#1aux1){};
}

% \newcommand{\exauxlinkint}[3]{%parametri: 1=box link, 2=x coordinate, 3=name link
% \node at (bangext-|#2)[etic](#1#3){\tiny $\aux$};
% }

\newcommand{\exauxlinkpos}[3]{%parametri: 1=box link, 2=auxposition, 3=name link
\node at (#2)[etic](#1#3){\tiny $\aux$};
}

\newcommand{\exaux}[2]{%parametri: 1=box link, 2=box right width
\node at (#1se.center)[left = (0.15*#2), etic](#1auxk){\tiny $\aux$};
\node at (#1se.center)[left=0.6*#2, etic](#1aux1){\tiny $\aux$};
}

\newcommand{\exauxcoo}[4]{%parametri: 1=box link, 2=box right width, 3=aux1 distance from right border, 4=aux1 distance from right border
\node at (#1se.center)[left = #4, etic](#1auxk){\tiny $\aux$};
\node at (#1auxk.center)[left=#3, etic](#1aux1){\tiny $\aux$};
}

\newcommand{\exauxports}[2]{%parametri: 1=box link, 2=box right width
\node at (#1se.center)[left = \stboxlw, etic](#1auxk){\tiny $\aux$};
\node at (#1auxk.center)[left=((#2)/2), etic](#1aux1){\tiny $\aux$};
\auxport{#1auxk}
\auxport{#1aux1}
}

\newcommand{\exauxportsg}[2]{%parametri: 1=box link, 2=box right width
\node at (#1se.center)[left = \stboxlw, nospace](#1auxk){};
\node at (#1auxk.center)[left=((#2)/2), nospace](#1aux1){};
\auxport{#1auxk}
\auxport{#1aux1}
}

\newcommand{\exauxportsglabm}[4]{%parametri: 1=box link, 2=box right width, 3=left lab, 4=right lab
\node at (#1se.center)[left = \stboxlw, nospace](#1auxk){};
\node at (#1auxk.center)[left=#2, nospace](#1aux1){};
\auxportlab{#1auxk}{below:#4}
\auxportlab{#1aux1}{below:#3}
}


\newcommand{\exauxportsglab}[4]{%parametri: 1=box link, 2=box right width, 3=left lab, 4=right lab
\node at (#1se.center)[left = \stboxlw, nospace](#1auxk){};
\node at (#1auxk.center)[left=((#2)/2), nospace](#1aux1){};
\auxportlab{#1auxk}{below:#4}
\auxportlab{#1aux1}{below:#3}
}
\newcommand{\exauxportsglabp}[5]{%parametri: 1=box link, 2=box right width, 3=left lab, 4=right lab, 5=line
\node at (#1se.center)[left = \stboxlw, nospace](#1auxk){};
\node at (#1auxk.center)[left=((#2)/2), nospace](#1aux1){};
\auxportlabp{#1auxk}{below:#4}{#5}
\auxportlabp{#1aux1}{below:#3}{#5}
}

\newcommand{\exauxportsglabpr}[5]{%parametri: 1=box link, 2=box right width, 3=left lab, 4=right lab, 5=line
\node at (#1se.center)[left = \stboxlw, nospace](#1auxk){};
\node at (#1auxk.center)[left=((#2)/2), nospace](#1aux1){};
\auxportlabp{#1auxk}{below right:#4}{#5}
\auxportlabp{#1aux1}{below right:#3}{#5}
}


\newcommand{\exauxportsglabshift}[5]{%parametri: 1=box link, 2=box right width, 3=left lab, 4=right lab 5=shift
\node at (#1se.center)[left = \stboxlw +#5, nospace](#1auxk){};
\node at (#1auxk.center)[left=((#2)/2), nospace](#1aux1){};
\auxportlab{#1auxk}{below:#4}
\auxportlab{#1aux1}{below:#3}
}

\newcommand{\auxnodes}[6]{%parametri: 1=box link, 2=distance between aux ports, 3=left lab, 4=right lab 5=shift, 6=distance ports from box
\node at (#1se.center)[left = \stboxlw +#5, nospace](#1auxk){};
\node at (#1auxk.center)[left=#2, nospace](#1aux1){};
\auxportnolinklabdist{#1auxk}{below:#4}{#6}
\auxportnolinklabdist{#1aux1}{below:#3}{#6}
}

\newcommand{\boxaux}[3]{%parametri: 1=box link, 2= box right width, 3=box kind
\ifthenelse{\equal{#3}{jbox}}{\jaux{#1}{#2}}{\exaux{#1}{#2}};
}

\newcommand{\boxlineNL}[1]{%parametri: #1=box link
\begin{pgfonlayer}{background layer} 
\draw[jboxline](#1.center) -- (#1no.center) -- (#1so.center) -- (#1se.center) -- (#1ne.center)--(#1.center); 
\end{pgfonlayer}
}
\newcommand{\boxnodesNL}[4]{%parametri: #1=Larghezza box destra, %#2= altezza box, #3=link to box, 4=larghezza sinistra
\node at (#3.center)[dummynode, left = #4](#3no){};
\node at (#3.center)[dummynode, right = #1](#3ne){};
\node at (#3ne.center)[dummynode, below=#2](#3se){};
\node at (#3se-|#3no)[dummynode](#3so){};
}

\newcommand{\stboxNL}[2]{%parameters: 1=link to box, 2=label
\boxNL{#1}{#2}{\stboxrw}{\stboxh}
}

\newcommand{\boxNL}[4]{%parameters: 1=link to box, 2=label, 3=larghezza, 4=altezza
\node at (#1.center)[dummynode, below=\sepbox](#1b){};
\boxnodesNL{#3}{#4}{#1b}{\stboxlw}
\node at \med{#1bno}{#1bse}[etic](#1blab){{\scriptsize #2}};
\boxlineNL{#1b}
}


\newcommand{\boxlineNR}[1]{%parametri: #1=box link
\begin{pgfonlayer}{background layer} 
\draw[jboxline](#1.center) -- (#1no.center) -- (#1so.center) -- (#1se.center) -- (#1ne.center)--(#1.center); 
\end{pgfonlayer}
}
\newcommand{\boxnodesNR}[4]{%parametri: #1=Larghezza box destra, %#2= altezza box, #3=link to box, 4=larghezza sinistra
\node at (#3.center)[dummynode, left = #1](#3no){};
\node at (#3.center)[dummynode, right = #4](#3ne){};
\node at (#3ne.center)[dummynode, below=#2](#3se){};
\node at (#3se-|#3no)[dummynode](#3so){};
}

\newcommand{\stboxNR}[2]{%parameters: 
\boxNR{#1}{#2}{\stboxrw}{\stboxh}
}

\newcommand{\boxNR}[4]{%parameters: 1=link to box, 2=label, 3=larghezza, 4=altezza
\node at (#1.center)[dummynode, below=\sepbox](#1b){};
\boxnodesNR{#3}{#4}{#1b}{\stboxlw}
\node at \med{#1bno}{#1bse}[etic](#1blab){{\scriptsize #2}};
\boxlineNL{#1b}
}

\newcommand{\boxlineol}[3]{%parametri: #1=box link, 2=line style, 3=jolly point on the left
%\begin{pgfonlayer}{background layer} 
\draw[#2](#1.center)--(#1se.center) -- (#1ne.center) -- (#1no.center) -- (#1so|-#3)--(#3.center)--(#3|-#1.center)--(#1.center); 
%\end{pgfonlayer}
}

\newcommand{\boxlineolol}[4]{%parametri: #1=box link, 2=line style, 3=jolly point on the left, 4= second jolly poin
%\begin{pgfonlayer}{background layer} 
\draw[#2](#1.center)--(#1se.center) -- (#1ne.center) -- (#1no.center) -- (#1so|-#4)--(#4.center)--(#4|-#3)--(#3.center)--(#3|-#1.center)--(#1.center); 
%\end{pgfonlayer}
}


\newcommand{\boxlineor}[3]{%parametri: #1=box link, 2=line style, 3=jolly point on the right
%\begin{pgfonlayer}{background layer} 
\draw[#2, overlay](#1.center) -- (#1-|#3)--(#3.center)--(#3-|#1se.center)--(#1ne.center) -- (#1no.center) -- (#1so.center)--(#1.center); 
%\end{pgfonlayer}
}

\newcommand{\boxlineorol}[4]{%parametri: #1=box link, 2=line style, 3=right jolly point, 4=left jolly point
%\begin{pgfonlayer}{background layer} 
\draw[#2, overlay](#1.center) -- (#1-|#3)--(#3.center)--(#3-|#1se.center)--(#1ne.center) -- (#1no.center) -- (#1no|-#4)--(#4.center)--(#4|-#1so)--(#1.center); 
%\end{pgfonlayer}
}



%\newcommand{\aboxol}[6]{%parametri: #1=Larghezza box destra, %#2= altezza box, #3=link to box, #4=label, 5=larghezza sinistra, 6=jolly point on the left
%% \boxnodes{#1}{#2}{#3}{#5}
%% \boxlineol{#3}{jboxline}{#6}
%% \boxlabel{#3}{#4}
%}

\newcommand{\aboxol}[7]{%parameters: 1=link to box, 2=box kind, 3=box left width, 4=box right width, 5= box height, #6=label #7=jolly point
\boxnodes{#4}{#5}{#1}{#3}
\boxlineol{#1}{#2line}{#7}
\boxlabel{#1}{#6}
}

\newcommand{\aboxolol}[8]{%parameters: 1=link to box, 2=box kind, 3=box left width, 4=box right width, 5= box height, #6=label #7=jolly point #8=second jolly point
\boxnodes{#4}{#5}{#1}{#3}
\boxlineolol{#1}{#2line}{#7}{#8}
\boxlabel{#1}{#6}
}

\newcommand{\aboxor}[7]{%parameters: 1=link to box, 2=box kind, 3=box left width, 4=box right width, 5= box height, #6=label #7=jolly point
\boxnodes{#4}{#5}{#1}{#3}
\boxlineor{#1}{#2line}{#7}
\boxlabel{#1}{#6}
}

\newcommand{\aboxorol}[8]{%parameters: 1=link to box, 2=box kind, 3=box left width, 4=box right width, 5= box height, #6=label #7=right jolly point #8=left jolly point
\boxnodes{#4}{#5}{#1}{#3}
\boxlineorol{#1}{#2line}{#7}{#8}
\boxlabel{#1}{#6}
}


%\newcommand{\aboxor}[6]{%parametri: #1=Larghezza box destra, %#2= altezza box, #3=link to box, #4=label, 5=larghezza sinistra, 6=jolly point on the right
%\boxnodes{#1}{#2}{#3}{#5}
%\boxlineor{#3}{jboxline}{#6}
%\boxlabel{#3}{#4}
%}

\newcommand{\aexboxol}[6]{%parametri: #1=Larghezza box destra, %#2= altezza box, #3=link to box, #4=label, 5=larghezza sinistra, 6=jolly point on the left
\boxnodes{#1}{#2}{#3}{#5}
\boxlineol{#3}{exboxline}{#6}
\boxlabel{#3}{#4}
}

\newcommand{\aexboxor}[6]{%parametri: #1=Larghezza box destra, %#2= altezza box, #3=link to box, #4=label, 5=larghezza sinistra, 6=jolly point on the right
\boxnodes{#1}{#2}{#3}{#5}
\boxlineor{#3}{exboxline}{#6}
\boxlabel{#3}{#4}
}


==> macros/graphical-macros/generic-links-before-new-whyn-trees.tex <==
%%%%%%%%%%%%%%%%
%% AXIOM
%%%%%%%%%%%%%%%

\newcommand{\axnode}[5]{
% 1 = left port
% 2 = right port
% 3 = link name
% 4 = height
% 5 = label size
\node at ($(#1.center)!.5!(#2.center)$) [above = #4, etic] (#3){ #5$\ax$};}

\newcommand{\axedges}[5 ]{
% 1 = left port
% 2 = right port
% 3 = link name
% 4 = left edge line style
% 5 = right edge line style
\draw[#4, in=90, out=180] (#3) to (#1);
\draw[#5, in=90, out=0] (#3) to (#2);
}

\newcommand{\laxabstract}[7]{
% 1 = left port
% 2 = right port
% 3 = link name
% 4 = height
% 5 = label size
% 6 = left edge line style
% 7 = right edge line style
\axnode{#1}{#2}{#3}{#4}{#5}
\axedges{#1}{#2}{#3}{#6}{#7}
}

%%%%%%%%%%%%%%%%
%% ZERARY
%%%%%%%%%%%%%%%

\newcommand{\lzeroary}[5]{
% 1 = one principal port	
% 2 = name of the link
% 3 = link symbol
% 4 = distance link-node
% 5 = type of edge
\node at (#1.center) [above= #4, etic] (#2){#3};
\draw[#5] (#2) to (#1);}


%%%%%%%%%%%%%%%%
%% UNARY
%%%%%%%%%%%%%%%

\newcommand{\lunarysymbol}[4]{
% 1 = bottom port, 
% 2 = top port, 
% 3 = name of the link, 
% 4 = link symbol
\node at ($(#2.center) ! .5 ! (#1.center)$) [etic] (#3){ #4};
}

\newcommand{\lunary}[5]{
% 1 = principal port	
% 2 = auxiliary port
% 3 = name of the link
% 4 = link symbol
% 5 = edge line
\lunarysymbol{#1}{#2}{#3}{#4}

\draw[#5] (#2) to (#3);
\draw[#5] (#3) to (#1);
}


%%%%%%%%%%%%%%%%
%% BINARY
%%%%%%%%%%%%%%%

\newcommand{\lbinsym}[5]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
% 5 = link symbol
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [etic] (#4){#5};
}

\newcommand{\lbinedgesabove}[4]{
% 1 = left auxiliary port	
% 2 = right auxiliary port	
% 3 = name of the link
% 4 = edge type
\draw[#4, in=150, out=-90] (#1) to (#3);
\draw[#4, in=30, out=-90] (#2) to (#3);
}

\newcommand{\lbinary}[6]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
% 5 = link symbol
% 6 = edge type
\lbinsym{#1}{#2}{#3}{#4}{#5}

% upper edges of the link
\lbinedgesabove{#2}{#3}{#4}{#6}

\draw[#6] (#4) to (#1);
}


%%%%%%%%%%%%%%%%
%% BOXES
%%%%%%%%%%%%%%%

\newcommand{\stboxlw}{6pt}
\newcommand{\stboxh}{20pt}
\newcommand{\stboxrw}{30pt}
\newcommand{\stboxrwaux}{35pt}
\newcommand{\sepbox}{2pt}
\newcommand{\belowbox}{\stboxh+2*\sepbox+1pt}

\newcommand{\boxnodes}[4]{
% 1 = link to box
% 2 = left width
% 3 = right width 
% 4 = height
\node at (#1.center)[left = #2,nospace](#1so){};
\node at (#1.center)[right = #3,nospace](#1se){};
\node at (#1se.center)[above=#4,nospace](#1ne){};
\node at (#1ne-|#1so)[nospace](#1no){};}

\newcommand{\boxline}[2]{
% 1 = box link
% 2 = line style
\draw[#2](#1.center) -- (#1se.center) -- (#1ne.center) -- (#1no.center) -- (#1so.center)--(#1.center);}

\newcommand{\abox}[5]{
% 1 = link to box
% 2 = line style
% 3 = right width 
% 4 = left width
% 5 = height
\boxnodes{#1}{#3}{#4}{#5}
\boxline{#1}{#2line}}

\newcommand{\boxauxnodes}[3]{
% 1 = link to box
% 2 = distance of the right conclusion from SE corner
% 3 = distance between the two conclusions
\node at (#1se.center)[left = #2, nospace](#1auxk){};
\node at (#1auxk.center)[left= #3, nospace](#1aux1){};
}

% \newcommand{\boxauxnodes}[2]{
% % 1 = link to box
% % 2 = box right width
% \node at (#1se.center)[left = \stboxlw, nospace](#1auxk){};
% \node at (#1auxk.center)[left= ((#2)/2), nospace](#1aux1){};
% }

\newcommand{\boxauxnodeslab}[4]{
% 1 = link to box
% 2 = left label,
% 3 = right label,
% 4 = height delta
\node at (#1auxk.center)[below = #4,etic](#1auxktarget){\tiny #3};
\node at (#1aux1.center)[below = #4,etic](#1aux1target){\tiny #2};

\draw[nopol] (#1auxk) to (#1auxktarget);
\draw[nopol] (#1aux1) to (#1aux1target);
}

\newcommand{\boxlabel}[2]{
% 1 = box link
% 2 = label
\node at ($(#1so)!.5!(#1ne)$) {#2};
}

\newcommand{\boxlineor}[3]{
% 1 = box link
% 2 = line style
% 3 = jolly point on the right
\draw[#2, overlay](#1.center) -- (#1-|#3)--(#3.center)--(#3-|#1se.center)--(#1ne.center) -- (#1no.center) -- (#1so.center)--(#1.center);}


\newcommand{\aboxor}[7]{
% 1 = link to box
% 2 = box kind
% 3 = box left width
% 4 = box right width
% 5 = box height
% 6 = label 
% 7 = jolly point
\boxnodes{#1}{#3}{#4}{#5}
\boxlineor{#1}{#2line}{#7}
\boxlabel{#1}{#6}}


%%%%%%%%%%%%%%%%
%% CONTRACTION AND WHYNOT TREES
%%%%%%%%%%%%%%%

\newcommand{\whyntreeabstract}[3]{
% 1 = principal node
% 2 = base length/2
% 3 = height
\node at (#1.center) [above left = #2 and #3, nospace](#1leftvertex){};
\node at (#1.center) [above right = #2 and #3, nospace](#1rightvertex){};

\draw[exboxline](#1.center) -- (#1leftvertex.center) -- (#1rightvertex.center) -- (#1.center);

\node at (#1.center) [above=3*#2/5,nospace](#1label){\tiny $T_{\contrp}$};

\node at (#1.center) [above left = #2 and #3/3, nospace](#1centerleftvertex){};
\node at (#1.center) [above right = #2 and #3/3, nospace](#1centerrightvertex){};

% boxline up right
\node at (#1centerleftvertex.center) [below = #2/4, nospace](#1leftupboxrightnode){};
\node at (#1leftupboxrightnode.center) [left= 2*#3/3, nospace](#1leftupboxleftnode){};
\draw[exboxline](#1leftupboxrightnode)to(#1leftupboxleftnode);

% boxline left
\node at (#1centerrightvertex.center) [below left = #2/2 and #3/6, nospace](#1rightupboxrightnode){};
\node at (#1rightupboxrightnode.center) [right= 2*#3/3, nospace](#1rightupboxleftnode){};
\draw[exboxline](#1rightupboxrightnode)to(#1rightupboxleftnode);

% boxline below right
\node at (#1.center) [above = #2/4, nospace](#1leftdownboxrightnode){};
\node at (#1leftdownboxrightnode.center) [left= 2*#3/3, nospace](#1leftdownboxleftnode){};
\draw[exboxline](#1leftdownboxrightnode)to(#1leftdownboxleftnode);

}

\newcommand{\whyntree}[1]{
% 1 = principal node
\whyntreeabstract{#1}{1.3*\stalt}{1.2*\stlar}
}

\newcommand{\whyntreeleaves}[1]{
% 1 = principal node
\node at (#1rightvertex.center) [above=\hstalt, etic](#1der1){\tiny $\der$};
\node at (#1centerrightvertex.center) [above=\hstalt, etic](#1dern){\tiny $\der$};
\node at (#1leftvertex.center) [above=\hstalt, etic](#1weakn){\tiny $\weak$};
\node at (#1centerleftvertex.center) [above=\hstalt, etic](#1weak1){\tiny $\weak$};

\draw[nopol](#1der1) to (#1rightvertex);
\draw[nopol](#1dern) to (#1centerrightvertex);
\draw[nopol](#1weak1) to (#1centerleftvertex);
\draw[nopol](#1weakn) to (#1leftvertex);

\gdots{#1der1}{#1dern}{below = 2pt}
\gdots{#1weak1}{#1weakn}{below = 2pt}
}

\newcommand{\whyntreeleaveswithpremises}[1]{
% 1 = principal node
\node at (#1rightvertex.center) [above=\hstalt, etic](#1dern){\tiny $\der$};
\node at (#1centerrightvertex.center) [above=\hstalt, etic](#1der1){\tiny $\der$};
\node at (#1leftvertex.center) [above=\hstalt, etic](#1weak1){\tiny $\weak$};
\node at (#1centerleftvertex.center) [above=\hstalt, etic](#1weakn){\tiny $\weak$};

\draw[nopol](#1der1) to (#1centerrightvertex);
\draw[nopol](#1dern) to (#1rightvertex);
\draw[nopol](#1weak1) to (#1leftvertex);
\draw[nopol](#1weakn) to (#1centerleftvertex);

\gdots{#1der1}{#1dern}{below = 2pt}
\gdots{#1weak1}{#1weakn}{below = 2pt}

\node at (#1der1.center) [above=\hstalt, nospace](#1der1premise){};
\node at (#1dern.center) [above=\hstalt, nospace](#1dernpremise){};
\draw[nopol](#1der1premise) to (#1der1);
\draw[nopol](#1dernpremise) to (#1dern);
}


%%%%%%%%%%%%%%%%
%% BOX BORDERS
%%%%%%%%%%%%%%%
\newcommand{\boxdershorizontaldistance}{7pt}
\newcommand{\boxdersverticaldistance}{2pt}
\newcommand{\boxdersdots}{5pt}

\newcommand{\boxcornerright}[4]{
% 1 = position
% 2 = width
% 3 = heigt
% 4 = boxline

% internal box
\node at (#1.center)[left=#2, nospace](#1lineaso){};
\node at (#1.center)[above=#3, nospace](#1lineane){};
\draw[#4](#1lineaso.center) -- (#1.center) -- (#1lineane.center);

% internal box dotted extensions
\node at (#1lineaso.center)[left=\boxdersdots, nospace](#1lineasodotted){};
\node at (#1lineane.center)[above=\boxdersdots, nospace](#1lineanedotted){};
\draw[#4, densely dotted](#1lineaso)to(#1lineasodotted);
\draw[#4, densely dotted](#1lineane)to(#1lineanedotted);
}


\newcommand{\boxcornersright}[4]{
% 1 = position
% 2 = width
% 3 = heigt
% 4 = boxline
\node at (#1.center)[above right=2pt and 4pt, etic](#1dots){\tiny $...$};
\boxcornerright{#1}{#2}{#3}{#4}

% external box
\node at (#1.center)[below right=\boxdersverticaldistance and \boxdershorizontaldistance, nospace](#1linease2){};
\node at (#1lineaso.center)[below=\boxdersverticaldistance, nospace](#1lineaso2){};

\node at (#1lineane.center)[right=\boxdershorizontaldistance, nospace](#1lineane2){};
\draw[#4](#1lineaso2.center) -- (#1linease2.center) -- (#1lineane2.center);

% external box dotted extensions
\node at (#1lineaso2.center)[left=\boxdersdots, nospace](#1lineaso2dotted){};
\node at (#1lineane2.center)[above=\boxdersdots, nospace](#1lineane2dotted){};
\draw[#4, densely dotted](#1lineaso2)to(#1lineaso2dotted);
\draw[#4, densely dotted](#1lineane2)to(#1lineane2dotted);



}

\newcommand{\boxcornerleft}[4]{
% 1 = position
% 2 = width
% 3 = heigt
% 4 = boxline

% internal box
\node at (#1.center)[right=#2, nospace](#1lineaso){};
\node at (#1.center)[above=#3, nospace](#1lineane){};
\draw[#4](#1lineaso.center) -- (#1.center) -- (#1lineane.center);

% internal box dotted extensions
\node at (#1lineaso.center)[right=\boxdersdots, nospace](#1lineasodotted){};
\node at (#1lineane.center)[above=\boxdersdots, nospace](#1lineanedotted){};
\draw[#4, densely dotted](#1lineaso)to(#1lineasodotted);
\draw[#4, densely dotted](#1lineane)to(#1lineanedotted);
}

\newcommand{\boxcornersleft}[4]{
% 1 = position
% 2 = width
% 3 = heigt
% 4 = boxline

\node at (#1.center)[above left=2pt and 4pt, etic](#1dots){\tiny $...$};

\boxcornerleft{#1}{#2}{#3}{#4}

% external box
\node at (#1.center)[below left=\boxdersverticaldistance and \boxdershorizontaldistance, nospace](#1linease2){};
\node at (#1lineaso.center)[below=\boxdersverticaldistance, nospace](#1lineaso2){};

\node at (#1lineane.center)[left=\boxdershorizontaldistance, nospace](#1lineane2){};
\draw[#4](#1lineaso2.center) -- (#1linease2.center) -- (#1lineane2.center);

% external box dotted extensions
\node at (#1lineaso2.center)[right=\boxdersdots, nospace](#1lineaso2dotted){};
\node at (#1lineane2.center)[above=\boxdersdots, nospace](#1lineane2dotted){};
\draw[#4, densely dotted](#1lineaso2)to(#1lineaso2dotted);
\draw[#4, densely dotted](#1lineane2)to(#1lineane2dotted);



}


==> macros/graphical-macros/links-axioms-cuts.tex <==
%\newcommand{\altax}{7pt}
\newcommand{\altaxghost}{10pt}
\newcommand{\althole}{10pt}
\newcommand{\altholem}{6pt}
\newcommand{\altaxbig}{10pt}
\newcommand{\altcut}{5pt}
\newcommand{\altcutbig}{10pt}

%ABSTRACT AXIOMS

\newcommand{\axabedges}[5 ]{%parametri: 1= negative port, 2= positive port, 3= link , 4=angle towards#1, 5=angle towards#2
\draw[negln, in=90, out=#4] (#3) to (#1);
\draw[posnl, in=#5, out=90] (#2) to (#3);
}

\newcommand{\axabedgesm}[5 ]{%parametri: 1= negative port, 2= positive port, 3= link , 4=angle towards#1, 5=angle towards#2
\draw[negln, in=90, out=#4] (#3) to (#1);
\draw[posnl, in=#5, out=90] (#2) to (#3);
}

\newcommand{\axabedgesmb}[5 ]{%parametri: 1= negative port, 2= positive port, 3= link , 4=angle towards#1, 5=angle towards#2
\draw[negln, in=105, out=#4] (#3) to (#1);
\draw[posnl, in=#5, out=75] (#2) to (#3);
}


\newcommand{\axedgesnor}[3 ]{%parametri: 1= negative port, 2= positive port, 3= link , 4=angle towards#1, 5=angle towards#2
\axabedgesm{#1}{#2}{#3}{180}{-7}}

\newcommand{\axedgesrev}[3 ]{%parametri: 1= negative port, 2= positive port, 3= link , 4=angle towards#1, 5=angle towards#2
\axabedgesmb{#1}{#2}{#3}{0}{195}}

\newcommand{\abaxnode}[5]{%parametri: 1= negative port, 2= positive port, 3= link , 4=height, 5=label size
\node at ($(#1.center)!.5!(#2.center)$) [above = #4, etic] (#3){ #5$\ax$};}

\newcommand{\abholenodenp}[5]{%parametri: 1= negative port, 2= positive port, 3= link , 4=height, 5=label size
\node at ($(#1.center)!.5!(#2.center)$) [above = #4, etic] (#3){ #5$\hole$};}


\newcommand{\labax}[5]{%parametri:%#1= axiom negative port	%#2= axiom positive port	%#3= name of the link, #4= height, 5=label size
\abaxnode{#1}{#2}{#3}{#4}{#5}
\axedgesnor{#1}{#2}{#3}
}

\newcommand{\labaxrev}[5]{%parametri:%#1= axiom negative port	%#2= axiom positive port	%#3= name of the link, #4= height,5=label size
\abaxnode{#1}{#2}{#3}{#4}{#5}
\axedgesrev{#1}{#2}{#3}
}

%STANDARD AXIOMS
% \newcommand{\lax}[3]{%parametri:%#1= axiom negative port	%#2= axiom positive port	%#3= name of the link
% \labax{#1}{#2}{#3}{\altax}{\tiny}}

\newcommand{\laxrev}[3]{%parametri:
\labaxrev{#1}{#2}{#3}{\altax}{\tiny}}

%BIGAXIOMS
\newcommand{\laxbig}[3]{%parametri:%#1= axiom negative port	%#2= axiom positive port	%#3= name of the link
\labax{#1}{#2}{#3}{\altaxbig}{\tiny}}

\newcommand{\laxbigrev}[3]{%parametri:
\labaxrev{#1}{#2}{#3}{\altaxbig}{\tiny}}

%DISTANT AXIOMS
\newcommand{\laxdist}[4]{%parametri: 	%#1= axiom negative port 	%#2= axiom positive port 	%#3= name of the link 	%#4= height
\labax{#1}{#2}{#3}{#4}{\tiny}}

\newcommand{\laxrevdist}[4]{%parametri: 	%#1= axiom negative port 	%#2= axiom positive port 	%#3= name of the link 	%#4= height
\labaxrev{#1}{#2}{#3}{#4}{\tiny}}


\newcommand{\lpholennp}[5]{ 
%parametri: 1= n1, 2= nk, 3=positive node, 4= link, 5=height
\abholenodenp{#2} {#3}{#4}{#5}{\tiny }

\draw[negln, in=60, out=180] (#4) to (#1);
\draw[negln, in=90, out=180] (#4) to (#2);
\draw[posnl, in=0, out=90] (#3) to (#4);
\gdots{#1}{#2}{}
}

\newcommand{\lpholennpm}[5]{ 
%parametri: 1= n1, 2= nk, 3=positive node, 4= link, 5=height
\abholenodenp{#2} {#3}{#4}{#5}{\tiny }

\draw[negln, in=60, out=180] (#4) to (#1);
\draw[negln, in=90, out=180] (#4) to (#2);
\draw[posnl, in=-15, out=90, looseness=1.5, overlay] (#3) to (#4);
\gdots{#1}{#2}{}
}


%ABSTRACT CUT
\newcommand{\cutabedges}[5 ]{%parametri: 1= negative port, 2= positive port, 3= link , 4=angle towards#1, 5=angle towards#2
\draw[posln, in=-90, out=#4] (#3) to (#1);
\draw[negnl, in=#5, out=-90] (#2) to (#3);
}

\newcommand{\cutnpabedges}[3 ]{%parametri: 1= negative port, 2= positive port, 3= link 
\draw[negln, out=-90, in=180] (#1) to (#3);
\draw[posnl, out=0, in=-90] (#3) to (#2);
}
\newcommand{\cutpnabedges}[3 ]{%parametri: 1= negative port, 2= positive port, 3= link 
\draw[negln, out=-90, in=0] (#2) to (#3);
\draw[posnl, out=180, in=-90] (#3) to (#1);
}


\newcommand{\cutedgesnor}[3 ]{%parametri: 1= negative port, 2= positive port, 3= link , 4=angle towards#1, 5=angle towards#2
\cutabedges{#1}{#2}{#3}{180}{0}}

\newcommand{\cutedgesrev}[3 ]{%parametri: 1= negative port, 2= positive port, 3= link , 4=angle towards#1, 5=angle towards#2
\draw[negln, out=-90, in=0] (#1) to (#3);
\draw[posnl, out=180, in=-90] (#3) to (#2);
}

\newcommand{\abcutnode}[5]{%parametri: 1= negative port, 2= positive port, 3= link , 4=height, 5=label size
\node at ($(#1.center)!.5!(#2.center)$) [below = #4, etic] (#3){ #5$\cut$};
}

\newcommand{\labcutnp}[5]{%parametri:%#1= negative port	%#2= positive port	%#3= name of the link, #4= height, 5=label size
\abcutnode{#1}{#2}{#3}{#4}{#5}
\cutnpabedges{#1}{#2}{#3}
}

\newcommand{\labcutpn}[5]{%parametri:%#1= positive port	%#2= negative port	%#3= name of the link, #4= height, 5=label size
\abcutnode{#2}{#1}{#3}{#4}{#5}
\cutpnabedges{#1}{#2}{#3}
}

\newcommand{\labcut}[5]{%parametri:%#1= axiom negative port	%#2= axiom positive port	%#3= name of the link, #4= height, 5=label size
\abcutnode{#1}{#2}{#3}{#4}{#5}
\cutedgesnor{#1}{#2}{#3}
}

\newcommand{\labcutrev}[5]{%parametri:%#1= axiom negative port	%#2= axiom positive port	%#3= name of the link, #4= height,5=label size
\abcutnode{#1}{#2}{#3}{#4}{#5}
\cutedgesrev{#1}{#2}{#3}
}

%%%%hole




%STANDARD CUTS
\newcommand{\lcut}[3]{%parametri:%#1= negative port	%#2= positive port	%#3= name of the link
\labcut{#1}{#2}{#3}{\altcut}{\tiny}}

\newcommand{\lcutnp}[3]{%parametri:%#1= negative port	%#2= positive port	%#3= name of the link
\labcutnp{#1}{#2}{#3}{\altcut}{\tiny}}


\newcommand{\lcutpn}[3]{%parametri:%#1= positive port	%#2= negative port	%#3= name of the link
\labcutpn{#1}{#2}{#3}{\altcut}{\tiny}}



\newcommand{\lcutrev}[3]{%parametri:
\labcutrev{#1}{#2}{#3}{\altcut}{\tiny}}

%BIG CUTS
\newcommand{\lcutbig}[3]{%parametri:%#1= axiom negative port	%#2= axiom positive port	%#3= name of the link
\labcut{#1}{#2}{#3}{\altcutbig}{\tiny}}

\newcommand{\lcutbigrev}[3]{%parametri:
\labcutrev{#1}{#2}{#3}{\altcutbig}{\tiny}}

%DISTANT CUTS
\newcommand{\lcutnpdist}[4]{%parametri: #1= negative port #2=positive port #3=name of the link #4=height
\labcutnp{#1}{#2}{#3}{#4}{\tiny}}

\newcommand{\lcutpndist}[4]{%parametri:%#1= positive port	%#2= negative port	%#3= name of the link
\labcutpn{#1}{#2}{#3}{#4}{\tiny}}

\newcommand{\lcutdist}[4]{%parametri: 	%#1= axiom negative port 	%#2= axiom positive port 	%#3= name of the link 	%#4= height
\labcut{#1}{#2}{#3}{#4}{\tiny}}

\newcommand{\lcutrevdist}[4]{%parametri: 	%#1= axiom negative port 	%#2= axiom positive port 	%#3= name of the link 	%#4= height
\labcutrev{#1}{#2}{#3}{#4}{\tiny}}

%FIXED CUTS
\newcommand{\lcutnpdistfixp}[4]{%parametri:	1= negative port, 2= positive port, 3= link name, 4= height
\node at ($(#2)!.5!(#2-|#1)$) [below = #4, etic] (#3){{\tiny $\cut$}};
\cutnpabedges{#1}{#2}{#3}
}

\newcommand{\lcutpndistfixp}[4]{%parametri:	1= positive port, 2= negative port, 3= link name, 4= height
\node at ($(#1)!.5!(#1-|#2)$) [below = #4, etic] (#3){$\cut$};
\cutnpabedges{#1}{#2}{#3}
}

\newcommand{\lcutrevdistfixp}[4]{%parametri:	1= positive port, 2= negative port, 3= link name, 4= height
\node at ($(#1)!.5!(#1-|#2)$) [below = #4, etic] (#3){$\cut$};
\cutedgesrev{#1}{#2}{#3}
}

\newcommand{\lcutrevdistfixn}[4]{%parametri:	1= positive port, 2= negative port, 3= link name, 4= height
\node at ($(#2)!.5!(#2-|#1)$) [below = #4, etic] (#3){$\cut$};
\cutedgesrev{#1}{#2}{#3}
}

\newcommand{\lcutdistfixp}[4]{%parametri:	1= positive port, 2= negative port, 3= link name, 4= height
\node at ($(#1)!.5!(#1-|#2)$) [below = #4, etic] (#3){$\cut$};
\cutedgesnor{#1}{#2}{#3}
}

\newcommand{\lcutdistfixn}[4]{%parametri:	1= positive port, 2= negative port, 3= link name, 4= height
\node at ($(#2)!.5!(#2-|#1)$) [below = #4, etic] (#3){$\cut$};
\cutedgesnor{#1}{#2}{#3}
}





%%%STOP LINKS%%%

%Abstract Stops
\newcommand{\abstopnode}[5]{%parametri: 1= negative port, 2= positive port, 3= link , 4=height, 5=label size
\node at ($(#1.center)!.5!(#2.center)$) [below = #4, etic] (#3){ #5$\stop$};
}

\newcommand{\labstop}[5]{%parametri:%#1= axiom negative port	%#2= axiom positive port	%#3= name of the link, #4= height, 5=label size
\abstopnode{#1}{#2}{#3}{#4}{#5}
\cutedgesnor{#1}{#2}{#3}
}

\newcommand{\labstoprev}[5]{%parametri:%#1= axiom negative port	%#2= axiom positive port	%#3= name of the link, #4= height,5=label size
\abstopnode{#1}{#2}{#3}{#4}{#5}
\cutedgesrev{#1}{#2}{#3}
}

%STANDARD STOPS
\newcommand{\lstop}[3]{%parametri:%#1= axiom negative port	%#2= axiom positive port	%#3= name of the link
\labstop{#1}{#2}{#3}{\altcut}{\tiny};}

\newcommand{\lstoprev}[3]{%parametri:
\labstoprev{#1}{#2}{#3}{\altcut}{\tiny}}


==> macros/graphical-macros/links-binary-marked-nor.tex <==
\newcommand{\lbinNop}[5]{%parametri: 	%#1=  principal port	%#2= left auxiliary port	%#3= right auxiliary port	%#4= name of the link    %#5= actual link kind
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [above= .5pt, etic] (#4){#5};

%edges of the link
\draw[nodelink] (#2) to (#4);
\draw[nodelink] (#3) to (#4);
\draw[linknode] (#4) to (#1);
}

\newcommand{\lbinNor}[5]{%parametri:
	%#1=  principal port
	%#2= left auxiliary port
	%#3= right auxiliary port
	%#4= name of the link
    %#5= actual link kind
%link symbol
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [above= .5pt, etic] (#4){#5};

%edges of the link
\draw[nodelinkNor, out=-90, in=180] (#2) to (#4);
\draw[nodelinkNor, out=-90, in=0] (#3) to (#4);
\draw[linknodeNor] (#4) to (#1);
}

\newcommand{\lbinMark}[5]{%parametri:	%#1=  principal port	%#2= left auxiliary port	%#3= right auxiliary port	%#4= name of the link    %#5= actual link kind
%link symbol
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [above= .5pt, etic] (#4){#5};

%edges of the link
\draw[nodelinkNor, out=-90, in=180] (#2) to (#4);
\draw[nodelinkNor, out=-90, in=0] (#3) to (#4);
\draw[linknodeMark] (#4) to (#1);
}

==> macros/graphical-macros/links-binary.tex <==
\newcommand{\lbinsym}[5]{%parameters: 1=  principal port, 2= left auxiliary port, 3= right auxiliary port, 4= name of the link, 5=link symbol
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [etic] (#4){#5};
}

\newcommand{\lbinfixr}[5]{%parameters: 1=  principal port, 2= left auxiliary port, 3= right auxiliary port, 4= name of the link, 5=link symbol
\node at ($(#1.center) ! .5 ! (#3 -| #1)$) [below= 1pt, etic] (#4){#5};
}

\newcommand{\lbinfixl}[5]{%parameters: 1=  principal port, 2= left auxiliary port, 3= right auxiliary port, 4= name of the link, 5=link symbol
\node at ($(#1.center) ! .5 ! (#3 -| #2)$) [below= 1pt, etic] (#4){#5};
}

\newcommand{\lposbin}[5]{%parametri: %#1=  principal port 	%#2= left auxiliary port 	%#3= right auxiliary port 	%#4= name of the link     %#5= actual link kind
\lbinsym{#1}{#2}{#3}{#4}{#5}
%edges of the link
\lposbinedges{#1}{#2}{#3}{#4}
}

\newcommand{\lposbinedges}[4]
{%parametri:	%#1= principal port	%#2= left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link
\draw[posln,out=150, in=-75] (#4) to (#2);
\draw[posln,out=30, in=-105] (#4) to (#3);
\draw[posnl] (#1) to (#4);
}

\newcommand{\lposbinfixl}[5]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	%#5= actual link
\node at ($(#1.center) ! .5 ! (#2 -| #1)$) [etic] (#4){#5};
%edges of the link
\lposbinedges{#1}{#2}{#3}{#4}}

\newcommand{\lposbinfixr}[5]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	%#5= actual link
\node at ($(#1.center) ! .5 ! (#3 -| #1)$) [etic] (#4){#5};
%edges of the link
\lposbinedges{#1}{#2}{#3}{#4}}

\newcommand{\lposbindeltah}[6]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	%#5= actual link %#6 traslazione in basso espressa in pt
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [above= 1-#6pt, etic] (#4){#5};
%edges of the link
\lposbinedges{#1}{#2}{#3}{#4}}

\newcommand{\lposbinfixd}[6]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	%#5= actual link #6=distance from principal port
\node at (#1.center) [above=#6,etic] (#4){#5};
%edges of the link
\lposbinedges{#1}{#2}{#3}{#4}}

\newcommand{\ltens}[4]{%parametri:	%#1= tensor principal port	%#2= tensor left auxiliary port	%#3= tensor right auxiliary port	%#4= name of the link
\lposbin{#1}{#2}{#3}{#4}{$\otimes$}}

\newcommand{\lwith}[4]{%parametri:	%#1= with principal port	%#2= with left auxiliary port	%#3= with right auxiliary port	%#4= name of the link
\lposbin{#1}{#2}{#3}{#4}{$\with$}}

%%%%%%%%%%%%
%%%%%%%%%%%%
%%%NEGATIVES
%%%%%%%%%%%%
%%%%%%%%%%%%

\newcommand{\lbinedges}[5]
{%parametri:	%#1= principal port	%#2= left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link, 5=edge type
\draw[#5, in=150, out=-75] (#2) to (#4);
\draw[#5, in=30, out=-105] (#3) to (#4);
\draw[#5] (#4) to (#1);
}

\newcommand{\lbinedgesm}[5]
{%parametri:	%#1= principal port	%#2= left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link, 5=edge type
\draw[#5, in=135, out=-75] (#2) to (#4);
\draw[#5, in=45, out=-105] (#3) to (#4);
\draw[#5] (#4) to (#1);
}

\newcommand{\lnegbinedges}[4]
{%parametri:	%#1= principal port	%#2= left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link
\lbinedgesm{#1}{#2}{#3}{#4}{negnl}}

\newcommand{\lnegbin}[5]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	%#5= actual link
\lbinsym{#1}{#2}{#3}{#4}{#5}
%edges of the link
\lnegbinedges{#1}{#2}{#3}{#4}
}


\newcommand{\lnegbinfixl}[5]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	%#5= actual link
\node at ($(#1.center) ! .5 ! (#2 -| #1)$) [etic] (#4){#5};
%edges of the link
\lnegbinedges{#1}{#2}{#3}{#4}}

\newcommand{\lnegbinfixr}[5]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	%#5= actual link
\node at ($(#1.center) ! .5 ! (#3 -| #1)$) [etic] (#4){#5};
%edges of the link
\lnegbinedges{#1}{#2}{#3}{#4}}


\newcommand{\lnegbindeltah}[6]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	%#5= actual link %#6 traslazione in basso espressa in pt
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [above= 1-#6pt, etic] (#4){#5};
%edges of the link
\lnegbinedges{#1}{#2}{#3}{#4}}

\newcommand{\lnegbinfixd}[6]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	%#5= actual link #6=distance from principal port
\node at (#1.center) [above=#6,etic] (#4){#5};
%edges of the link
\lnegbinedges{#1}{#2}{#3}{#4}}



\newcommand{\lpar}[4]{%parametri:	%#1= par principal port	%#2= par left auxiliary port	%#3= par right auxiliary port	%#4= name of the link
\lnegbin{#1}{#2}{#3}{#4}{$\parr$}}


\newcommand{\lcontra}[4]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link
\lnegbin{#1}{#2}{#3}{#4}{$\curlyvee$}}

\newcommand{\lcontre}[4]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link
\lnegbin{#1}{#2}{#3}{#4}{$\contr$}}

\newcommand{\lcontrp}[4]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link
\lnegbin{#1}{#2}{#3}{#4}{$\contrp$}}

==> macros/graphical-macros/links-jumps.tex <==
\newcommand{\lajump}[3]{%parametri:	%#1= source	%#2= anchor	%#3=actual jump type
\draw [#3](#1)to (#2);}
%\draw [#3](#1)to node[etic,fill=white]{} (#2);}

\newcommand{\lajumpcoo}[6]{%parametri:	%#1= source	%#2= anchor	%3= out	%4= in	%5= looseness #6=actual jump type
\draw [#6, out= #3, in = #4, looseness=#5](#1) to (#2);}

\newcommand{\lajumpgen}[3]{%parametri:	%#1= source	%#2= anchor	%#3=actual jump type
\draw [#3gen](#1)to node[etic,fill=white]{} (#2);}

\newcommand{\lajumpgencoo}[6]{%parametri:	%#1= source	%#2= anchor	%3= out	%4= in	%5= looseness #6=actual jump type
\draw [#6gen, out= #3, in = #4, looseness=#5](#1) to (#2);}


\newcommand{\ljump}[2]{%parametri: %#1= source 	%#2= anchor 
\lajump{#1}{#2}{jumpshift}}

% \newcommand{\lejump}[2]{%parametri: %#1= source 	%#2= anchor 
% \lajump{#1}{#2}{\ej}}

\newcommand{\ljumpcoo}[5]{%parametri:	%#1= source 	%#2= anchor	%3= out	%4= in	%5= looseness
\lajumpcoo{#1}{#2}{#3}{#4}{#5}{jumpshift}}

% \newcommand{\lejumpcoo}[5]{%parametri:	%#1= source 	%#2= anchor	%3= out	%4= in	%5= looseness
% \lajumpcoo{#1}{#2}{#3}{#4}{#5}{\ej}}

% \newcommand{\ljumpbord}[2]{%parametri:	%#1= source	%#2= anchor
% \lajump{#1}{#2}{$\bord$}}

\newcommand{\ljumpcut}[2]{%parametri:	%#1= source	%#2= anchor
\lajump{#1}{#2}{jumpcut}}

\newcommand{\ljumpcutcoo}[5]{%parametri:	%#1= source	%#2= anchor	%3= out	%4= in	%5= looseness
\lajumpcoo{#1}{#2}{#3}{#4}{#5}{jumpcut}}

\newcommand{\ljumpbot}[2]{%parametri:	%#1= source	%#2= anchor
\lajump{#1}{#2}{jumpzero}}

\newcommand{\ljumpbotcoo}[5]{%parametri:	%#1= source	%#2= anchor	%3= out	%4= in	%5= looseness
\lajumpcoo{#1}{#2}{#3}{#4}{#5}{jumpzero}}

\newcommand{\ljumpbord}[2]{%parametri:	%#1= source	%#2= anchor
\lajump{#1}{#2}{jumpbord}}

\newcommand{\ljumpbordcoo}[5]{%parametri:	%#1= source	%#2= anchor	%3= out	%4= in	%5= looseness
\lajumpcoo{#1}{#2}{#3}{#4}{#5}{jumpbord}}

% \newcommand{\ljumpbordcoo}[5]{%parametri:	%#1= source	%#2= anchor	%3= out	%4= in	%5= looseness
% \lajumpcoo{#1}{#2}{#3}{#4}{#5}{$\bord$}}



==> macros/graphical-macros/links-lambda-calculus.tex <==
\newcommand{\llambin}[5]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	%#5= actual link
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [etic] (#4){#5};
%edges of the link
\draw[ln, out=165, in=-90] (#4) to (#2);
\draw[ln, out=15, in=-90] (#4) to (#3);
\draw[nl] (#1) to (#4);
}

\newcommand{\llambinneg}[5]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	%#5= actual link
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [etic] (#4){#5};
%edges of the link
\draw[negln, in=165, out=-90] (#2) to (#4);
\draw[negln, in=15, out=-90] (#3) to (#4);
\draw[negnl] (#4) to (#1);
}

\newcommand{\lvarn}[4]{%parametri:	%#1=  principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [etic] (#4){$\vop$};
%edges of the link
\draw[ln, out=150, in=-90] (#4) to (#2);
\draw[ln, out=30, in=-90] (#4) to (#3);
\draw[nl] (#1) to (#4);
\node at ($(#2)!.5!(#3)$) [etic]{\tiny $\ldots$};
}

\newcommand{\lvarweak}[2]{%parametri:	%#1=  principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	
\node at (#1.center) [above= \hstalt,etic] (#2){$\weakp$};
%edges of the link
\draw[negnl] (#2) to (#1);
}

\newcommand{\lvarweakgen}[2]{%parametri:	%#1=  principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	
\node at (#1.center) [above= \hstalt,etic] (#2){$\weakp$};
%edges of the link
\draw[negnlgen] (#2) to (#1);
}


\newcommand{\lsubab}[4]{%parametri:	%#1=  principal port	%#2= auxiliary port	%#3= name of the link, actual link	
\node at \med{#2}{#1} [etic] (#3){\scriptsize #4};

\draw[linknode] (#3) to (#2);
\draw[posnl] (#1) to (#3);
}
% \newcommand{\lsub}[3]{%parametri:	%#1=  principal port	%#2= auxiliary port	%#3= name of the link	
% \lsubab{#1}{#2}{#3}{$[\cdot]$}
% }

\newcommand{\lvarder}[3]{%parametri:	%#1=  principal port	%#2= auxiliary port	%#3= name of the link	
\node at ($(#2.center) ! .5 ! (#1.center)$) [etic] (#3){\scriptsize $\vop$};

\draw[negln] (#2) to (#3);
\draw[negnl] (#3) to (#1);
}

\newcommand{\lvarderout}[4]{%parametri:	%#1=  principal port	%#2= auxiliary port	%#3= name of the link #4=out degree	
\node at ($(#2.center) ! .5 ! (#2|-#1)$) [etic] (#3){\scriptsize $\vop$};

\draw[negln] (#2) to (#3);
\draw[negnl, out=-90, in=#4] (#3) to (#1);
}


\newcommand{\lvarcontr}[4]{%parametri:	%#1= par principal port	%#2= par left auxiliary port	%#3= par right auxiliary port	%#4= name of the link
\llambinneg{#1}{#2}{#3}{#4}{$\vop$}}




\newcommand{\labs}[4]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link	
\node at ($(#1.center) ! .5 ! (#3 -| #1)$) [below= 1pt, etic] (#4){$\l$};
%edges of the link
\draw[posln, out=-90, in=90] (#1) to (#4);
\draw[negnl, in=210, out=90] (#2) to (#4);
\draw[posnl, out=-30, in=90] (#4) to (#3);
}

\newcommand{\labsweak}[4]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link	
\node at ($(#1.center) ! .5 ! (#3 -| #1)$) [below= 1pt, etic] (#4){$\l$};
%edges of the link
\draw[posln, out=-90, in=90] (#1) to (#4);
\draw[negln, in=210, out=60] (#2) to (#4);
\draw[posnl, out=-30, in=90] (#4) to (#3);
}

\newcommand{\labsangle}[7]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link %#5=out of binding edge #6=in of binding edge #7=looseness
\node at ($(#1.center) ! .5 ! (#3 -| #1)$) [below= 1pt, etic] (#4){$\l$};
%edges of the link
\draw[posln, out=-90, in=90] (#1) to (#4);
\draw[negnl, in=#5, out=#6, looseness=#7] (#2) to (#4);
\draw[posnl, out=-30, in=90] (#4) to (#3);
}

\newcommand{\labsangles}[5]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link %#5=parametri binding edge
\node at ($(#1.center) ! .5 ! (#3 -| #1)$) [below= 1pt, etic] (#4){$\l$};
%edges of the link
\draw[posln, out=-90, in=90] (#1) to (#4);
\draw[negnl, #5] (#2) to (#4);
\draw[posnl, out=-30, in=90] (#4) to (#3);
}

\newcommand{\lap}[4]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link	
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [below= 1pt, etic] (#4){@};
%edges of the link
\draw[posln, in=90, out=-90] (#1) to (#4);
\draw[posnl, in=90, out=210] (#4) to (#2);
\draw[posnl, in=90, out=-30] (#4) to (#3);
}

\newcommand{\lhole}[4]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link	
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [below= 1pt, etic] (#4){$\square$};
%edges of the link
\draw[negln, in=90, out=-90] (#1) to (#4);
\draw[negnl, in=90, out=210] (#4) to (#2);
\draw[negnl, in=90, out=-30] (#4) to (#3);

}

\newcommand{\lholev}[4]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link	
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [below= 1pt, etic] (#4){$\vop$};
%edges of the link
\draw[negln, in=90, out=-90] (#1) to (#4);
\draw[negnl, in=90, out=210] (#4) to (#2);
\draw[negnl, in=90, out=-30] (#4) to (#3);
\gdots{#2}{#3}{}
}

\newcommand{\lholen}[4]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link	
\lhole{#1}{#2}{#3}{#4}
\gdots{#2}{#3}{}
}


\newcommand{\lvarcoln}[4]{%parametri:	%#1=  principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [etic] (#4){$\vop$};
%edges of the link
\draw[posln, out=180, in=-90] (#4) to (#2);
\draw[posln, out=0, in=-90] (#4) to (#3);
\draw[nodelink] (#1) to (#4);
\node at ($(#2)!.5!(#3)$) [etic]{\tiny $\ldots$};
}

\newcommand{\lvarcol}[4]{%parametri:	%#1=  principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [etic] (#4){$\vop$};
%edges of the link
\draw[ln, out=180, in=-90] (#4) to (#2);
\draw[ln, out=0, in=-90] (#4) to (#3);
\draw[nl] (#1) to (#4);
}

\newcommand{\lvarcolfixl}[4]{%parametri:	%#1=  principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	
\node at \med{#1.center}{\med{#2.center}{#2-|#3}.center}[etic] (#4){$\vop$};
%edges of the link
\draw[ln, out=180, in=-90] (#4) to (#2);
\draw[ln, out=0, in=-90] (#4) to (#3);
\draw[nl] (#1) to (#4);
}




%%%%%%%%%%%ù
%%%%%%%%%ùùùù
%%%%%%%%%%%ù
\newcommand{\lvarbinfixl}[4]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	
\node at ($(#1.center) ! .5 ! (#2 -| #1)$) [etic] (#4){$\vop$};
%edges of the link
\draw[negln, in=165, out=-90] (#2) to (#4);
\draw[negln, in=15, out=-90] (#3) to (#4);
\draw[negnl] (#4) to (#1);

}

\newcommand{\lvarbinfixr}[4]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	
\node at ($(#1.center) ! .5 ! (#3 -| #1)$) [etic] (#4){$\vop$};
%edges of the link
\draw[negln, in=165, out=-90] (#2) to (#4);
\draw[negln, in=15, out=-90] (#3) to (#4);
\draw[negnl] (#4) to (#1);
}


\newcommand{\lvarbindeltah}[6]{%parametri:	%#1= contra principal port	%#2= contra left auxiliary port	%#3= contra right auxiliary port	%#4= name of the link	%#6 traslazione in basso espressa in pt
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [above= 1-#6pt, etic] (#4){$\vop$};
%edges of the link
\draw[negln, in=165, out=-90] (#2) to (#4);
\draw[negln, in=15, out=-90] (#3) to (#4);
\draw[negnl] (#4) to (#1);
}


==> macros/graphical-macros/links-mixedbinary.tex <==
\newcommand{\larrowabs}[5]{%parametri: %#1=  principal port 	%#2= left auxiliary port 	%#3= right auxiliary port 	%#4= name of the link     %#5= actual link kind
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [above= .5pt, etic] (#4){#5};
%edges of the link
\draw[linknode,out=180, in=-90] (#4) to (#2);
\draw[nodelink,out=-90, in=0] (#3) to (#4);
\draw[linknode] (#4) to (#1);
}

\newcommand{\larrowl}[5]{%parametri: %#1=  principal port 	%#2= left auxiliary port 	%#3= right auxiliary port 	%#4= name of the link
\larrowabs{#1}{#2}{#3}{#4}{$\limp$}
}

\newcommand{\lsubtrl}[5]{%parametri: %#1=  principal port 	%#2= left auxiliary port 	%#3= right auxiliary port 	%#4= name of the link
\lsubtrabs{#1}{#2}{#3}{#4}{$\subtrl$}
}

\newcommand{\lsubtrabs}[5]{%parametri: %#1=  principal port 	%#2= left auxiliary port 	%#3= right auxiliary port 	%#4= name of the link     %#5= actual link kind
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [above= .5pt, etic] (#4){#5};

%edges of the link
\draw[nodelink,out=-90, in=180] (#2) to (#4);
\draw[linknode,out=0, in=-90] (#4) to (#3);
\draw[nodelink] (#1) to (#4);
}


==> macros/graphical-macros/links-namenets.tex <==

\newcommand{\lparn}[4]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
\lBinaryWithEdgeBelowTypes{#1}{#2}{#3}{#4}{{\scriptsize$\parr$}}{mprincnpar,purenRev}{exppuren}{purenRev}
}

\newcommand{\lparnfake}[4]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
\lBinSymbol{#1}{#2}{#3}{#4}{}
}

%
\newcommand{\lparnangle}[5]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
% 5 = binding edge parameters

% symbol
\lBinSymbolFixR{#1}{#2}{#3}{#4}{$\parr$}

% edges
\draw[exppuren, #5] (#2) to (#4);
\draw[puren, out=-30, in=90] (#4) to (#3);
\draw[mprincn, puren] (#1) to (#4);
}

\newcommand{\lparnanglefake}[5]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
% 5 = binding edge parameters
\lBinSymbolFixR{#1}{#2}{#3}{#4}{}
}

%
\newcommand{\ltensn}[4]{
% 1 = principal port	
% 2 = left auxiliary port	
% 3 = right auxiliary port	
% 4 = name of the link
\lBinaryWithEdgeBelowTypes{#1}{#2}{#3}{#4}{$\tens$}{purenRev}{purenRev}{exppurenRev}
\draw[mprincn,puren, out=210, in=90] (#4) to (#2);
}
%
\newcommand{\lbangn}[3]{
% 1 = bottom port, 
% 2 = top port, 
% 3 = name of the link
\lUnaryDiffEdges{#1}{#2}{#3}{\scriptsize $!$}{puren}{eprincn, exppuren}
}

\newcommand{\lbangnfake}[3]{
% 1 = bottom port, 
% 2 = top port, 
% 3 = name of the link
\lUnarySymbol{#1}{#2}{#3}{\scriptsize $!$}
}


\newcommand{\ldern}[3]{
% 1 = bottom port, 
% 2 = top port, 
% 3 = name of the link
\lUnaryDiffEdges{#1}{#2}{#3}{\scriptsize $\der$}{eprincn, exppuren}{puren}
}

\newcommand{\ldernangle}[4]{
% 1 = bottom port, 
% 2 = top port, 
% 3 = name of the link
% 4 = angle
\node at ($(#2.center) ! .5 ! (#2 |- #1)$) [above= .5pt,fill=white, etic] (#3){\scriptsize $\der$};
\draw[puren] (#2) to (#3);
\draw[eprincn, exppuren, #4] (#3) to (#1);
%\draw[ exppure, #4] (#3) to (#1);
%\node at (#1.center)[below =1pt, nospace](#4point){};
}


%\newcommand{\lpurederout}[4]
%{%parametri: %#1=  bottom port 	%#2= top port 	%#3= link name = angle
%\node at ($(#2.center) ! .5 ! (#2|-#1)$) [above= .5pt,fill=white, etic] (#3){\scriptsize $\der$};
%
%\draw[pure] (#2) to (#3);
%\draw[princ, exppure, out=-90,in=#4] (#3) to (#1);
%%\node at (#1.center)[below =1pt, nospace](#4point){};
%}
%
\newcommand{\lweakn}[2]
{%parametri: %#1=  principal port 	%#2= left auxiliary port 	%#3= right auxiliary port 	%#4= name of the link     %#5= actual link kind
\node at (#1.center) [above= \hstalt,fill=white, etic] (#2){\scriptsize$\weak$};

\draw[eprincn, revexppuren] (#2) to (#1);

%\node at (#1.center)[below =1pt, nospace](#4point){};
}
%
\newcommand{\lcolboxn}[4]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link	

\lBinaryWithEdgeBelowTypes{#1}{#2}{#3}{#4}{$\ctxhole$}{purenRev}{exppurenRev}{exppurenRev}

%\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [below= 1pt, etic] (#4){$\square$};
%%edges of the link
%\draw[pure, in=90, out=-90] (#1) to (#4);
%\draw[exppure, in=90, out=210] (#4) to (#2);
%\draw[exppure, in=90, out=-30] (#4) to (#3);

}
%
%\newcommand{\lpholeb}[4]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link	
%\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [below= 1pt, etic] (#4){$\square^!$};
%%edges of the link
%\draw[exppure, in=90, out=-90] (#1) to (#4);
%\draw[exppure, in=90, out=210] (#4) to (#2);
%\draw[exppure, in=90, out=-30] (#4) to (#3);
%
%}
%
%\newcommand{\lpholebn}[4]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link	
%\lpholeb{#1}{#2}{#3}{#4}
%\gdots{#2}{#3}{}
%}
%
%\newcommand{\lpholeln}[4]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link	
%\lpholel{#1}{#2}{#3}{#4}
%\gdots{#2}{#3}{}
%}


%
%\newcommand{\lzeroarynopol}[3]{%parametri: %#1=  bottom port	%#2= name of the link     %#3= actual link kind
%\node at (#1.center) [above= \hstalt,fill=white, etic] (#2){\scriptsize#3};
%
%\draw[nopol] (#1) to (#2);
%}
%
%\newcommand{\lunarynopolangle}[5]{%parametri: %#1=  bottom port 	%#2= top port 	%#3= name of the link     %#4= actual link kind, 5=angle on bottom port
%\node at ($(#2.center) ! .5 ! (#2|-#1)$) [etic] (#3){\scriptsize #4};
%\draw[nopol] (#3) to (#2);
%\draw[nopol,out=#4, in=-90] (#1) to (#3);
%}
%
%\newcommand{\lbinarynopol}[5]
%{%parametri: %#1=  principal port 	%#2= left auxiliary port 	%#3= right auxiliary port 	%#4= name of the link     %#5= actual link kind
%\lbinsym{#1}{#2}{#3}{#4}{#5}
%\draw[nopol, out=210, in=90] (#4) to (#2);
%\draw[nopol, out=-30, in=90] (#4) to (#3);
%\draw[nopol] (#1) to (#4);
%}
%

==> macros/graphical-macros/links-nopol.tex <==
%VARIATIONS
\newcommand{\laxNop}[3]{%parametri:	%#1= axiom negative port 	%#2= axiom positive port 	%#3= name of the link
\abaxnode{#1}{#2}{#3}{\altax}{\tiny}
%edges of the link
\draw[nopol, out=180, in=90] (#3) to (#1);
\draw[nopol, out=0, in=90] (#3) to (#2);
}

\newcommand{\laxNor}[3]{%parametri: 	%#1= axiom negative port	%#2= axiom positive port	%#3= name of the link
\abaxnode{#1}{#2}{#3}{\altax}{\tiny}
%edges of the link
\draw[nopol, out=180, in=90] (#3) to (#1);
\draw[nopol, out=0, in=90] (#3) to (#2);
}

\newcommand{\laxNorp}[3]{%parametri: 	%#1= axiom negative port	%#2= axiom positive port	%#3= name of the link
\abaxnode{#1}{#2}{#3}{\altax}{\tiny}
%edges of the link
\draw[nopolrev, out=180, in=90] (#3) to (#1);
\draw[nopol, out=0, in=90] (#3) to (#2);
}

\newcommand{\laxMark}[3]{%parametri: 	%#1= axiom negative port 	%#2= axiom positive port 	%#3= name of the link
\abaxnode{#1}{#2}{#3}{\altax}{\tiny}
%edges of the link
\draw[linknodeMark, out=180, in=90] (#3) to (#1);
\draw[linknodeMark, out=0, in=90] (#3) to (#2);
}

\newcommand{\laxNordist}[4]{%parametri: 	%#1= axiom negative port 	%#2= axiom positive port 	%#3= name of the link 	%#4= vertical distance of the link symbol from the nodes
\node at ($(#1.center)!.5!(#2.center)$) [above = #4, etic] (#3){\tiny$\ax$};
%edges of the link
\draw[nopol, out=180, in=90] (#3) to (#1);
\draw[nopol, out=0, in=90] (#3) to (#2);
}
\newcommand{\laxNorpdist}[4]{%parametri: 	%#1= axiom negative port 	%#2= axiom positive port 	%#3= name of the link 	%#4= vertical distance of the link symbol from the nodes
\node at ($(#1.center)!.5!(#2.center)$) [above = #4, etic] (#3){\tiny$\ax$};
%edges of the link
\draw[nopolrev, out=180, in=90] (#3) to (#1);
\draw[nopol, out=0, in=90] (#3) to (#2);
}

\newcommand{\lcutNop}[3]{%parametri:%#1= cut positive port	%#2= cut negative port	%#3= name of the link
%link symbol
\abcutnode{#1}{#2}{#3}{\altcut}{\tiny}

%edges of the link
\draw[nopol, out=-90, in=180] (#1) to (#3);
\draw[nopol, out=-90, in=0] (#2) to (#3);
}

\newcommand{\lcutNor}[3]{%parametri:	%#1= cut positive port	%#2= cut negative port	%#3= name of the link

%link symbol
\abcutnode{#1}{#2}{#3}{\altcut}{\tiny}

%edges of the link
\draw[nopol, out=-90, in=180] (#1) to (#3);
\draw[nopol, out=-90, in=0] (#2) to (#3);
}

\newcommand{\lcutNorp}[3]{%parametri:	%#1= cut positive port	%#2= cut negative port	%#3= name of the link

%link symbol
\abcutnode{#1}{#2}{#3}{\altcut}{\tiny}

%edges of the link
\draw[nopolrev, out=-90, in=180] (#1) to (#3);
\draw[nopol, out=-90, in=0] (#2) to (#3);
}

\newcommand{\lcutNordist}[4]{%parametri:	%#1= cut positive port	%#2= cut negative port	%#3= name of the link, 4=distance

%link symbol
\abcutnode{#1}{#2}{#3}{#4}{\tiny}

%edges of the link
\draw[nopol, out=-90, in=180] (#1) to (#3);
\draw[nopol, out=-90, in=0] (#2) to (#3);
}
\newcommand{\lcutNorpdist}[4]{%parametri:	%#1= cut positive port	%#2= cut negative port	%#3= name of the link, 4=distance

%link symbol
\abcutnode{#1}{#2}{#3}{#4}{\tiny}

%edges of the link
\draw[nopolrev, out=-90, in=180] (#1) to (#3);
\draw[nopol, out=-90, in=0] (#2) to (#3);
}

\newcommand{\lcutNordistfixp}[4]{%parametri:	%#1= cut positive port	%#2= cut negative port	%#3= name of the link, 4=distance

%link symbol
\node at ($(#2)!.5!(#2-|#1)$) [below = #4, etic] (#3){\tiny$\cut$};

%edges of the link
\draw[nopol, out=-90, in=180] (#1) to (#3);
\draw[nopol, out=-90, in=0] (#2) to (#3);
}



\newcommand{\lbinNop}[5]{%parametri: 	%#1=  principal port	%#2= left auxiliary port	%#3= right auxiliary port	%#4= name of the link    %#5= actual link kind
\lbinsym{#1}{#2}{#3}{#4}{#5}

%edges of the link
\draw[nopol] (#2) to (#4);
\draw[nopol] (#3) to (#4);
\draw[nopol] (#4) to (#1);
}

\newcommand{\lbin}[6]{%parametri:	%#1=  principal port	%#2= left auxiliary port	%#3= right auxiliary port	%#4= name of the link    %#5= actual link kind, 6= line kind
%link symbol
\lbinsym{#1}{#2}{#3}{#4}{#5}

%edges of the link
\lbinedges{#1}{#2}{#3}{#4}{#6}
}


\newcommand{\lbinNor}[5]{%parametri:	%#1=  principal port	%#2= left auxiliary port	%#3= right auxiliary port	%#4= name of the link    %#5= actual link kind
%link symbol
\lbinsym{#1}{#2}{#3}{#4}{#5}

%edges of the link
\lbinedges{#1}{#2}{#3}{#4}{nopol}
}

\newcommand{\lbinNorp}[5]{%parametri:	%#1=  principal port	%#2= left auxiliary port	%#3= right auxiliary port	%#4= name of the link    %#5= actual link kind
%link symbol
\lbinsym{#1}{#2}{#3}{#4}{#5}

%edges of the link
\lbinedges{#1}{#2}{#3}{#4}{nopolrev}
}

\newcommand{\lbinNorfixd}[6]{%parametri:	%#1=  principal port	%#2= left auxiliary port	%#3= right auxiliary port	%#4= name of the link    %#5= actual link kind, 6=distance
%link symbol
\node at (#1.center) [above=#6,etic] (#4){#5};

%edges of the link
\lbinedges{#1}{#2}{#3}{#4}{nopol}
}



\newcommand{\lparNor}[4]{%parametri:	%#1=  principal port	%#2= left auxiliary port	%#3= right auxiliary port	%#4= name of the 
\lbinNor{#1}{#2}{#3}{#4}{$\parr$}
}
\newcommand{\ltensNor}[4]{%parametri:	%#1=  principal port	%#2= left auxiliary port	%#3= right auxiliary port	%#4= name of the 
\lbinNor{#1}{#2}{#3}{#4}{$\otimes$}
}
\newcommand{\lcontrNor}[4]{%parametri:	%#1=  principal port	%#2= left auxiliary port	%#3= right auxiliary port	%#4= name of the 
\lbinNor{#1}{#2}{#3}{#4}{$\contr$}
}

\newcommand{\lcontrpNor}[4]{%parametri:	%#1=  principal port	%#2= left auxiliary port	%#3= right auxiliary port	%#4= name of the 
\lbinNor{#1}{#2}{#3}{#4}{$\DSubs$}
}

\newcommand{\lbinNorgen}[5]{%parametri:	%#1=  principal port	%#2= left auxiliary port	%#3= right auxiliary port	%#4= name of the link    %#5= actual link kind
%link symbol
\lbinsym{#1}{#2}{#3}{#4}{#5}

%edges of the link
\lbinedges{#1}{#2}{#3}{#4}{gengray, nopol}
}

\newcommand{\lunaNor}[4]{%parametri:	%#1=  bottom port	%#2= top port	 #3= name of the link    #4= actual link kind
%link symbol
\lunasym{#1}{#2}{#3}{#4}

%edges of the link
\draw[nopol] (#2) to (#3);
\draw[nopol] (#3) to (#1);

}
\newcommand{\lderNor}[3]{%parametri:	%#1=  bottom port	%#2= top port	 #3= name of the link    #4= actual link kind
\lunaNor{#1}{#2}{#3}{$\der$}
}
\newcommand{\lbangNor}[3]{%parametri:	%#1=  bottom port	%#2= top port	 #3= name of the link    #4= actual link kind
\lunaNor{#1}{#2}{#3}{$!$}
}
\newcommand{\lbangNorfixd}[3]{%parametri: %#1=  principal port 	%#2= auxiliary port  #3=name of the link  ;
\node at (#1.center) [above= \hstalt, etic] (#3){\scriptsize !};

\draw[nopolrev] (#1) to (#3);
\draw[nopol] (#2) to (#3);
%\draw[posln, #5] (#4) to (#3);
}


\newcommand{\lbinMark}[5]{%parametri:	%#1=  principal port	%#2= left auxiliary port	%#3= right auxiliary port	%#4= name of the link    %#5= actual link kind
%link symbol
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [above= .5pt, etic] (#4){#5};

%edges of the link
\draw[nodelinkNor, out=-90, in=180] (#2) to (#4);
\draw[nodelinkNor, out=-90, in=0] (#3) to (#4);
\draw[linknodeMark] (#4) to (#1);
}

\newcommand{\lzeroNor}[3]{%parametri: 	%#1= one principal port	%#2= name of the link, 3=actual link
\node at (#1.center) [above= \hstalt, etic] (#2){\scriptsize #3};
\draw[nopol] (#2) to (#1);}

\newcommand{\lzeroNorrev}[3]{%parametri: 	%#1= one principal port	%#2= name of the link, 3=actual link
\node at (#1.center) [above= \hstalt, etic] (#2){\scriptsize #3};
\draw[nopolrev] (#2) to (#1);}

\newcommand{\lbotNor}[2]{%parametri: 	%#1= one principal port	%#2= name of the link, 
\lzeroNor{#1}{#2}{$\bot$}
}

\newcommand{\loneNor}[2]{%parametri: 	%#1= one principal port	%#2= name of the link, 
\lzeroNor{#1}{#2}{$1$}
}

\newcommand{\loneNorrev}[2]{%parametri: 	%#1= one principal port	%#2= name of the link, 
\lzeroNorrev{#1}{#2}{$1$}
}

\newcommand{\lweakNor}[2]{%parametri: 	%#1= one principal port	%#2= name of the link, 
\lzeroNor{#1}{#2}{$\weak$}
}
\newcommand{\lweakpNor}[2]{%parametri: 	%#1= one principal port	%#2= name of the link, 
\lzeroNor{#1}{#2}{$\wop$}
}

\newcommand{\lzeroNordist}[4]{%parametri: 	%#1= one principal port	%#2= name of the link, 3= distance, 4=actual link
\node at (#1.center) [above= #3, etic] (#2){\scriptsize #4};
\draw[nopol] (#2) to (#1);}

\newcommand{\lpholenNor}[5]{ 
%parametri: 1= n1, 2= nk, 3=positive node, 4= link, 5=height
\abholenodenp{#2} {#3}{#4}{#5}{\tiny }

\draw[nopol, in=60, out=180] (#4) to (#1);
\draw[nopol, in=90, out=180] (#4) to (#2);
\draw[nopolrev, in=0, out=90] (#3) to (#4);
\gdots{#1}{#2}{}
}

\newcommand{\lpholenNorrev}[5]{ 
%parametri: 1= n1, 2= nk, 3=positive node, 4= link, 5=height
\abholenodenp{#2} {#3}{#4}{#5}{\tiny }

\draw[nopol, in=120, out=0] (#4) to (#1);
\draw[nopol, in=90, out=0] (#4) to (#2);
\draw[nopolrev, in=180, out=90] (#3) to (#4);
\gdots{#1}{#2}{}
}

\newcommand{\lpholenNorrevp}[5]{ 
%parametri: 1= n1, 2= nk, 3=positive node, 4= link, 5=height
\abholenodenp{#2} {#3}{#4}{#5}{\tiny }

\draw[nopol, in=120, out=0] (#4) to (#1);
\draw[nopol, in=90, out=0] (#4) to (#2);
\draw[nopol, in=180, out=90] (#3) to (#4);
\gdots{#1}{#2}{}
}

\newcommand{\lderNorcg}[3]{%parametri:	%#1= abup principal port	%#2= abup auxiliary port	%#3= name of the link
\node at ($(#1.center)!.5!(#2.center)$) [fill=white,etic] (#3){\scriptsize $\der$};
\draw[nopol] (#3) to (#1);
\draw[nopol] (#3) to (#2);
}
\newcommand{\lbangNorcg}[3]{%parametri:	%#1= down principal port	%#2= down auxiliary port	%#3= name of the link
\node at ($(#1.center)!.5!(#2.center)$) [fill=white,etic] (#3){\scriptsize$!$};
\draw[nopol] (#1) to (#3);
\draw[nopol] (#2) to (#3);
}



==> macros/graphical-macros/links-purenets.tex <==

\newcommand{\lzeroarynopol}[3]{%parametri: %#1=  bottom port	%#2= name of the link     %#3= actual link kind
\node at (#1.center) [above= \hstalt,fill=white, etic] (#2){\scriptsize#3};

\draw[nopol] (#1) to (#2);
}

\newcommand{\lunarynopolangle}[5]{%parametri: %#1=  bottom port 	%#2= top port 	%#3= name of the link     %#4= actual link kind, 5=angle on bottom port
\node at ($(#2.center) ! .5 ! (#2|-#1)$) [etic] (#3){\scriptsize #4};
\draw[nopol] (#3) to (#2);
\draw[nopol,out=#4, in=-90] (#1) to (#3);
}

\newcommand{\lbinarynopol}[5]
{%parametri: %#1=  principal port 	%#2= left auxiliary port 	%#3= right auxiliary port 	%#4= name of the link     %#5= actual link kind
\lbinsym{#1}{#2}{#3}{#4}{#5}
\draw[nopol, out=210, in=90] (#4) to (#2);
\draw[nopol, out=-30, in=90] (#4) to (#3);
\draw[nopol] (#1) to (#4);
}

\newcommand{\lpurepar}[4]
{%parametri: %#1=  principal port 	%#2= left auxiliary port 	%#3= right auxiliary port 	%#4= name of the link     %#5= actual link kind
%\lbinarynopol{#1}{#2}{#3}{#4}{$\parr$}
\lbinsym{#1}{#2}{#3}{#4}{$\parr$}
%\node at (#1.center)[below =1pt, nospace](#4point){};
\draw[exppure, in=210, out=90] (#2) to (#4);
\draw[pure, out=-30, in=90] (#4) to (#3);
\draw[princ,pure] (#1) to (#4);
}

\newcommand{\lpureparangle}[5]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link %#5=binding edge parameters
\lbinfixr{#1}{#2}{#3}{#4}{$\parr$}
%edges of the link
\draw[exppure, #5] (#2) to (#4);
\draw[pure, out=-30, in=90] (#4) to (#3);
\draw[princ, pure] (#1) to (#4);
}

\newcommand{\lpuretens}[4]
{%parametri: %#1=  principal port 	%#2= left auxiliary port 	%#3= right auxiliary port 	%#4= name of the link     %#5= actual link kind
\lbinsym{#1}{#2}{#3}{#4}{$\otimes$}
%\node at (#1.center)[below =1pt, nospace](#4point){};
\draw[princ,pure, out=210, in=90] (#4) to (#2);
\draw[exppure, out=-30, in=90] (#4) to (#3);
\draw[pure] (#1) to (#4);

%\node at (#1.center)[below =1pt, nospace](#4point){};
}

\newcommand{\lpurebang}[3]
{%parametri: %#1=  bottom port 	%#2= top port 	%#3= link name
\node at ($(#2.center) ! .5 ! (#1.center)$) [above= .5pt,fill=white, etic] (#3){\scriptsize $!$};

\draw[princ, exppure] (#2) to (#3);
\draw[pure] (#3) to (#1);
%\node at (#1.center)[below =1pt, nospace](#4point){};
}

\newcommand{\lpureder}[3]
{%parametri: %#1=  bottom port 	%#2= top port 	%#3= link name
\node at ($(#2.center) ! .5 ! (#1.center)$) [above= .5pt,fill=white, etic] (#3){\scriptsize $\der$};

\draw[pure] (#2) to (#3);
\draw[princ, exppure] (#3) to (#1);
%\node at (#1.center)[below =1pt, nospace](#4point){};
}
\newcommand{\lpurederout}[4]
{%parametri: %#1=  bottom port 	%#2= top port 	%#3= link name = angle
\node at ($(#2.center) ! .5 ! (#2|-#1)$) [above= .5pt,fill=white, etic] (#3){\scriptsize $\der$};

\draw[pure] (#2) to (#3);
\draw[princ, exppure, out=-90,in=#4] (#3) to (#1);
%\node at (#1.center)[below =1pt, nospace](#4point){};
}

\newcommand{\lpureweak}[2]
{%parametri: %#1=  principal port 	%#2= left auxiliary port 	%#3= right auxiliary port 	%#4= name of the link     %#5= actual link kind
\node at (#1.center) [above= \hstalt,fill=white, etic] (#2){\scriptsize$\weak$};

\draw[princ, exppure] (#2) to (#1);

%\node at (#1.center)[below =1pt, nospace](#4point){};
}

\newcommand{\lpholel}[4]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link	
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [below= 1pt, etic] (#4){$\square$};
%edges of the link
\draw[pure, in=90, out=-90] (#1) to (#4);
\draw[exppure, in=90, out=210] (#4) to (#2);
\draw[exppure, in=90, out=-30] (#4) to (#3);

}

\newcommand{\lpholeb}[4]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link	
\node at ($(#2.center) ! .5 ! (#3.center) ! .5 ! (#1.center)$) [below= 1pt, etic] (#4){$\square^!$};
%edges of the link
\draw[exppure, in=90, out=-90] (#1) to (#4);
\draw[exppure, in=90, out=210] (#4) to (#2);
\draw[exppure, in=90, out=-30] (#4) to (#3);

}

\newcommand{\lpholebn}[4]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link	
\lpholeb{#1}{#2}{#3}{#4}
\gdots{#2}{#3}{}
}

\newcommand{\lpholeln}[4]{%parametri:	%#1=  output	%#2= left below port	%#3= right below port	%#4= name of the link	
\lpholel{#1}{#2}{#3}{#4}
\gdots{#2}{#3}{}
}


==> macros/graphical-macros/links-shifts.tex <==
\newcommand{\lupcorgr}[3]{%parametri:	%#1= up principal port	%#2= up auxiliary port	%#3= name of the link
\node at ($(#1.center)!.5!(#2.center)$) [etic] (#3){$\su$};
\draw[nodelink] (#1) to (#3);
\draw[linknode] (#3) to (#2);
}


\newcommand{\labup}[4]{%parametri:	%#1= abup principal port	%#2= abup auxiliary port	%#3= name of the link	%#4= actual link
\node at ($(#1.center)!.5!(#2.center)$) [fill=white,etic] (#3){#4};
\draw[negnl] (#3) to (#1);
\draw[posnl] (#3) to (#2);
}

\newcommand{\lup}[3]{%parametri:	%#1= up principal port	#2= up auxiliary port 	%#3= name of the link
\labup{#1}{#2}{#3}{$\up$}}


\newcommand{\lderp}[3]{%parametri:	%#1= up principal port	%#2= up auxiliary port	%#3= name of the link
\labup{#1}{#2}{#3}{$\der$}}


\newcommand{\ldown}[3]{%parametri: 	%#1= down principal port 	%#2= down auxiliary port	%#3= name of the link
\labdown{#1}{#2}{#3}{$\down$}}

\newcommand{\lbangp}[3]{%parametri:	%#1= up principal port	%#2= up auxiliary port	%#3= name of the link
\labdown{#1}{#2}{#3}{$!$}}

\newcommand{\labdown}[4]{%parametri:	%#1= down principal port	%#2= down auxiliary port	%#3= name of the link	%#4= actual link
\node at ($(#1.center)!.5!(#2.center)$) [fill=white,etic] (#3){#4};
\draw[posln] (#1) to (#3);
\draw[negnl] (#2) to (#3);
}

\newcommand{\labdowncor}[4]{%parametri:	%#1= down principal port	%#2= down auxiliary port	%#3= name of the link	%#4= actual link
\node at ($(#1.center)!.5!(#2.center)$) [etic] (#3){#4};
\draw[posln] (#3) to (#1);
%\draw[linknode] (#3) to (#2);
}


==> macros/graphical-macros/links-unary.tex <==
\newcommand{\lunasym}[4]{%parameters: 1=  bottom port, 2= top port, 3= name of the link, 4=link symbol
\node at ($(#2.center) ! .5 ! (#1.center)$) [etic] (#3){\scriptsize #4};
}

\newcommand{\lunadown}[4]{%parameters: 1=  bottom port, 2= top port, 3= name of the link, 4=link symbol
\node at (#1.center) [above=\hstalt, etic] (#3){\scriptsize #4};
}

\newcommand{\lposunary}[5]{%parametri: %#1=  principal port 	%#2= auxiliary port 	%#4= name of the link     %#5= actual link kind
\lunasym{#1}{#2}{#3}{#4}

\draw[posnl] (#2) to (#3);
\draw[posln] (#3) to (#1);
}

\newcommand{\lnegunary}[4]{%parametri: %#1=  principal port 	%#2= auxiliary port 	%#4= name of the link     %#5= actual link kind
\lunasym{#1}{#2}{#3}{#4}

\draw[negln] (#3) to (#2);
\draw[negnl] (#1) to (#3);
}

\newcommand{\laux}[3]{
\lnegunary{#1}{#2}{#3}{$\aux$}
}

\newcommand{\lauxfromports}[1]{
\node at (#1.center) [above= \hstalt,negport] (#1pab){};
\node at (#1.center) [below= \hstalt,negport] (#1pbe){};
\draw[negln] (#1) to (#1pab);
\draw[negnl] (#1pbe) to (#1);
}

\newcommand{\lauxfromportslab}[3]{
\node at (#1.center) [above= \hstalt,label=#2,negport] (#1pab){};
\node at (#1.center) [below= \hstalt,label=#3,negport] (#1pbe){};
\draw[negln] (#1) to (#1pab);
\draw[negnl] (#1pbe) to (#1);
}


\newcommand{\lplusr}[3]{
\lnegunary{#1}{#2}{#3}{\tiny$\plusr$}
}

\newcommand{\lplusl}[3]{
\lnegunary{#1}{#2}{#3}{\tiny$\plusl$}
}

\newcommand{\lposf}[3]{
\lposunary{#1}{#2}{#3}{$\posf$}
}

\newcommand{\lnegf}[3]{
\lnegunary{#1}{#2}{#3}{$\negf$}
}


\newcommand{\lder}[3]{
\lnegunary{#1}{#2}{#3}{$\der$}
}

\newcommand{\ldig}[3]{
\lnegunary{#1}{#2}{#3}{$\dig$}
}

\newcommand{\lders}[5]{%parametri: %#1=  principal port 	%#2= auxiliary port #3=star node %#4= name of the link #5=star parameters;
\node at ($(#2.center) ! .5 ! (#1.center)$) [above= .5pt,fill=white, etic] (#4){\scriptsize$\der$};

\draw[posln] (#4) to (#2);
\draw[negln] (#4) to (#1);
\draw[posnl, #5](#3)to(#4);
}

\newcommand{\ldersl}[4]{%parametri: %#1=  principal port 	%#2= auxiliary port #3=star node %#4= name of the link
\lders{#1}{#2}{#3}{#4}{in=210, out=75}}


\newcommand{\ldersr}[4]{%parametri: %#1=  principal port 	%#2= auxiliary port #3=star node %#4= name of the link
\lders{#1}{#2}{#3}{#4}{in=-30, out=105}}

\newcommand{\lbangs}[5]{%parametri: %#1=  principal port 	%#2= auxiliary port  #3=star port %#4= name of the link  #5=star parameters;
\lunasym{#1}{#2}{#4}{!}

\draw[posnl] (#1) to (#4);
\draw[negln] (#2) to (#4);
\draw[posln, #5] (#4) to (#3);
}

\newcommand{\lbangsfixd}[5]{%parametri: %#1=  principal port 	%#2= auxiliary port  #3=star port %#4= name of the link  #5=star parameters;
\node at (#1.center) [above= \hstalt, etic] (#4){\scriptsize !};

\draw[posnl] (#1) to (#4);
\draw[negln] (#2) to (#4);
\draw[posln, #5] (#4) to (#3);
}



\newcommand{\lbangpfixd}[3]{%parametri: %#1=  principal port 	%#2= auxiliary port  #3=name of the link  ;
\node at (#1.center) [above= \hstalt, etic] (#3){\scriptsize !};

\draw[posnl] (#1) to (#3);
\draw[negln] (#2) to (#3);
%\draw[posln, #5] (#4) to (#3);
}
\newcommand{\lderpfixd}[3]{%parametri: %#1=  principal port 	%#2= auxiliary port  #3=name of the link  ;
\node at (#1.center) [above= \hstalt+1pt, etic] (#3){\scriptsize $\der$};

\draw[negln] (#3) to (#1);
\draw[posnl] (#3) to (#2);
%\draw[posln, #5] (#4) to (#3);
}

\newcommand{\lbangsl}[4]{%parametri: %#1=  principal port 	%#2= auxiliary port  #3=star port %#4= name of the link  
\lbangs{#1}{#2}{#3}{#4}{in=-75, out=150}}


\newcommand{\lbangsr}[4]{%parametri: %#1=  principal port 	%#2= auxiliary port  #3=star port %#4= name of the link  
\lbangs{#1}{#2}{#3}{#4}{in=-105, out=30}}


==> macros/graphical-macros/links-zeroary.tex <==
\newcommand{\lone}[2]{%parametri: 	%#1= one principal port	%#2= name of the link
\node at (#1.center) [above= \hstalt, etic] (#2){\scriptsize 1};
\draw[posnl] (#1) to (#2);}

\newcommand{\lonem}[2]{%parametri: 	%#1= one principal port	%#2= name of the link
\node at (#1.center) [above= \hstaltm, etic] (#2){\scriptsize 1};
\draw[posnl] (#1) to (#2);}

\newcommand{\lonebig}[2]{%parametri: 	%#1= one principal port	%#2= name of the link
\node at (#1.center) [above= \hstaltbig, etic] (#2){1};
\draw[posnl] (#1) to (#2);}


\newcommand{\lonedist}[3]{%parametri:	%#1= one principal port	%#2= name of the link	%#3= distance link-node
\node at (#1.center) [above= #3, etic] (#2){1};
\draw[posnl] (#1) to (#2);}

\newcommand{\lnegzero}[3]{%parametri:	%#1= one principal port	%#2= name of the link	%#3=actual link
\node at (#1.center) [above= \hstalt, etic] (#2){\scriptsize#3};
\draw[negln] (#2) to (#1);}

\newcommand{\lnegzerom}[3]{%parametri:	%#1= one principal port	%#2= name of the link	%#3=actual link
\node at (#1.center) [above= \hstaltm, etic] (#2){\scriptsize#3};
\draw[negln] (#2) to (#1);}

\newcommand{\lnegzerop}[5]{%parametri:	%#1= one principal port	%#2= name of the link	%#3=actual link #4=relative position 5#=edge degrees
\node at (#1.center) [#4, etic] (#2){\scriptsize#3};
\draw[negln, #5] (#2) to (#1);}

\newcommand{\lnegzerobig}[3]{%parametri:	%#1= one principal port	%#2= name of the link	%#3=actual link
\node at (#1.center) [above= \hstaltbig, etic] (#2){#3};
\draw[negln] (#2) to (#1);}


\newcommand{\lbot}[2]{%parametri:	%#1= one principal port	%#2= name of the link
\lnegzero{#1}{#2}{$\bot$}}

\newcommand{\lweak}[2]{%parametri:%#1= one principal port	%#2= name of the link
\lnegzero{#1}{#2}{$\weak$}}

\newcommand{\lweakm}[2]{%parametri:%#1= one principal port	%#2= name of the link
\lnegzerom{#1}{#2}{$\weakp$}}

\newcommand{\lweakp}[2]{%parametri:%#1= one principal port	%#2= name of the link
\lnegzero{#1}{#2}{$\weakp$}}

\newcommand{\lauxz}[2]{%parametri:%#1= aux principal port	%#2= name of the link
\lnegzero{#1}{#2}{$\aux$}}


\newcommand{\auxport}[1]{%parametri:%#1= aux link 
\auxportnolink{#1}
\draw[negnl] (#1) to (#1port);}

\newcommand{\auxportlab}[2]{%parametri:%#1= aux link, 2=port label
\auxportnolinklab{#1}{#2}
\draw[negnl] (#1) to (#1port);}

\newcommand{\auxportp}[2]{%parametri:%#1= aux link, 2=line
\auxportnolink{#1}
\draw[#2] (#1) to (#1port);}

\newcommand{\auxportlabp}[3]{%parametri:%#1= aux link, 2=port label, 3=line
\node at (#1.center) [below= \hstalt, label =#2, port] (#1port){};
\draw[#3] (#1) to (#1port);}


\newcommand{\auxportnolinklab}[2]{%parametri:%#1= aux link, 2=port label
\auxportnolinklabdist{#1}{#2}{\hstalt}
}

\newcommand{\auxportnolinklabdist}[3]{%parametri:%#1= aux link, 2=port label, 3=distance from box
\node at (#1.center) [below= #3, label =#2, negport] (#1port){};
}

\newcommand{\auxportnolink}[1]{%parametri:%#1= aux link
\auxportnolinklab{#1}{below:}
}


\newcommand{\lbotdist}[3]{%parametri:	%#1= one principal port	%#2= name of the link	%#3= distance link-node
\node at (#1.center) [above= #3, etic] (#2){$\bot$};
\draw[negln] (#2) to (#1);}

\newcommand{\labdum}[3]{%parametri: 1= dum aux port, 2= name of the link, 3=actual link,
\node at (#1.center)[below=\hstalt, etic](#2){\scriptsize #3};
\draw[linknode] (#2) to (#1);}

\newcommand{\ldum}[2]{%parametri: 1= dum aux port, 2= name of the link, 
\labdum{#1}{#2}{$\dummy$}}

